ReasonCLIP-58M: Visually Grounded Commonsense Reasoning Supervision for CLIP

CLIP and its variants are widely adopted visual backbones in multimodal systems, but their pretraining remains dominated by descriptive image-text alignment. As downstream applications increasingly demand visually grounded commonsense inference and compositional reasoning, it remains unclear whether CLIP-style encoders can support such reasoning without architectural changes. To address this, we present ReasonCLIP-58M, a continual pretraining framework that integrates large-scale reasoning supervision into CLIP-style models through our two-stage strategy, which progressively integrates reasoning signals while preserving descriptive alignment, followed by category-structured reasoning supervision. To support this framework, we construct two complementary datasets and a benchmark: ReasonLite-42M, with open-form, visually verifiable reasoning captions; ReasonPro-16M, with category-specific reasoning supervision; and RCLIP-Bench for diagnostic evaluation of visually grounded reasoning. We train a family of ReasonCLIP that improves visually grounded commonsense and compositional reasoning while also enhancing zero-shot retrieval performance. As a drop-in visual encoder for multimodal large language models such as LLaVA-NeXT, ReasonCLIP delivers consistent gains without additional inference cost, demonstrating that structured reasoning supervision enhances the expressive capacity of CLIP-style visual representations. All datasets, models, and training code are available at https://github.com/RISys-Lab/ReasonCLIP.

==> sec/0-abs.tex <==
\begin{abstract}
CLIP and its variants are widely adopted visual backbones in multimodal systems, but their pretraining remains dominated by descriptive image-text alignment. As downstream applications increasingly demand visually grounded commonsense inference and compositional reasoning, it remains unclear whether CLIP-style encoders can support such reasoning without architectural changes.
% \NL{Refining on progress.}
% To address this, we present \textbf{ReasonCLIP-58M}, a reasoning-oriented continual pretraining framework that integrates large-scale visually grounded commonsense supervision into CLIP-style models through a two-stage, non-intrusive training strategy. Stage 1 performs reasoning-aware alignment through joint descriptive and reasoning supervision, while Stage 2 introduces explicit category-level reasoning signals to promote structured representation learning. 
% To support this framework, we construct two complementary datasets: ReasonLite-42M, which provides open-form, visually verifiable reasoning captions, and ReasonPro-16M, which offers category-specific supervision across five reasoning types. We further introduce RCLIP-Bench, a hierarchical diagnostic benchmark that evaluates visual grounding, evidence awareness, and structured reasoning.
% Using our framework, we train reasoning-enhanced encoders that consistently improve visually grounded commonsense and compositional reasoning, and yield gains in zero-shot retrieval. When integrated as a drop-in visual backbone for multimodal large language models such as LLaVA, ReasonCLIP delivers stable downstream improvements without additional inference cost. These results demonstrate that structured reasoning supervision substantially expands the expressive capacity of CLIP-style visual representations. All datasets, models, and training code will be publicly released.
% To address this, we introduce ReasonCLIP-58M, a family of CLIP-style visual encoders trained via a two-stage continual framework over 58.9M visually grounded commonsense reasoning samples. The first stage incrementally integrates reasoning signals to preserve descriptive alignment, while the second stage introduces structured category-level supervision to enforce discrimination among reasoning patterns. To support this framework, we construct ReasonLite-42M with open-form, visually verifiable reasoning captions and ReasonPro-16M with category-specific supervision across five reasoning types. We further introduce RCLIP-Bench, a diagnostic benchmark for visually grounded reasoning. Across diverse CLIP and SigLIP backbones, ReasonCLIP not only improves visually grounded commonsense and compositional reasoning but also enhances zero-shot retrieval performance. As a drop-in encoder for multimodal large language models such as LLaVA, it yields consistent downstream gains without additional inference cost, demonstrating that structured reasoning supervision expands the expressive capacity of CLIP-style visual representations.
To address this, we present ReasonCLIP-58M, a continual pretraining framework that integrates large-scale reasoning supervision into CLIP-style models through our two-stage strategy, which progressively integrates reasoning signals while preserving descriptive alignment, followed by category-structured reasoning supervision.
% that disentangles reasoning enhancement from preserving descriptive alignment. % and explicit reasoning supervision. 
To support this framework, we construct two complementary datasets and a benchmark: ReasonLite-42M, with open-form, visually verifiable reasoning captions; ReasonPro-16M, with category-specific reasoning supervision; and RCLIP-Bench for diagnostic evaluation of visually grounded reasoning. We train a family of ReasonCLIP that improves visually grounded commonsense and compositional reasoning while also enhancing zero-shot retrieval performance. 
As a drop-in visual encoder for multimodal large language models such as LLaVA-NeXT, ReasonCLIP delivers consistent gains without additional inference cost, % \BZ{:}\st{downstream} gains without additional inference cost,
% When used as a drop-in encoder in multimodal large language models, such as LLaVA, ReasonCLIP delivers consistent downstream improvements without additional inference cost,
demonstrating that structured reasoning supervision enhances the expressive capacity of CLIP-style visual representations.
All datasets, models, and training code will be publicly released.

% CLIP and its variants are widely adopted visual backbones in multimodal systems, yet their pretraining objective primarily focuses on descriptive image–text alignment. As downstream applications demand commonsense inference and compositional understanding, it remains unclear whether such encoders can natively support visual reasoning without architectural modification. To address this gap, we present ReasonCLIP-58M, a continual pretraining framework that injects large-scale commonsense reasoning supervision into CLIP-style models. Our approach employs a progressive multi-stage strategy that decouples reasoning enhancement from alignment preservation, enabling stable integration of reasoning into the existing representation space. We further construct ReasonLite-42M with open-form visually verifiable reasoning captions, ReasonPro-16M with category-specific supervision across five perception-grounded reasoning types, and RCLIP-Bench, a diagnostic benchmark for visually grounded reasoning. Evaluated on diverse CLIP and SigLIP backbones across model scales, ReasonCLIP improves commonsense and compositional reasoning while yielding gains in zero-shot retrieval. As a drop-in encoder for multimodal systems such as LLaVA and SDXL, it delivers stable downstream improvements without additional inference cost, demonstrating that structured reasoning supervision expands the expressive capacity of CLIP-style visual representations. All datasets, models, and training scripts will be released publicly.

% CLIP and its variants have become widely adopted visual backbones in multimodal systems, yet their pretraining objective remains largely confined to descriptive image–text alignment. As downstream applications increasingly demand commonsense inference and compositional understanding, it is unclear whether CLIP-style encoders can be extended to natively support visual reasoning without architectural modification. We present ReasonCLIP-58M, a continual pretraining framework that introduces large-scale commonsense supervision while preserving its alignment capability. Our approach employs a progressive multi-stage training strategy that decouples reasoning enhancement from alignment preservation, 
% enabling stable integration of reasoning into the existing representation space.
% % allowing structured reasoning patterns to emerge within the original representation space without disrupting its learned semantics. 
% To support this framework, we construct ReasonLite-42M with open-form visually verifiable reasoning captions, ReasonPro-16M with category-specific supervision across five perception-grounded reasoning types, and RCLIP-Bench as a diagnostic benchmark for visually grounded reasoning. Evaluated on diverse CLIP and SigLIP backbones across model scales, ReasonCLIP consistently improves commonsense and compositional reasoning while also achieving gains in zero-shot retrieval. When used as a drop-in encoder in multimodal systems such as LLaVA and SDXL, it delivers stable downstream improvements without additional inference cost, demonstrating that structured reasoning supervision can effectively expand the expressive capacity of CLIP-style visual representations. All datasets, models, and training scripts will be released publicly.


% CLIP and its variants have become widely adopted visual foundation models in multimodal systems, yet their pretraining objectives are largely limited to descriptive image-text alignment. 
% %
% \SC{What Reasoning?}
% As multimodal systems increasingly demand reasoning capabilities, the potential of CLIP-style visual encoders to support such capabilities remains underexplored. 
% %
% \SC{add R-CLIP} 
% In this work, we propose ReasonCLIP, a non-intrusive continual pretraining framework that enhances reasoning capability while preserving descriptive alignment, built upon two automatically constructed datasets, ReasonLite-42M and ReasonPro-16M, organized under a progressive multi-stage training strategy.
% %
% We train multiple CLIP and SigLIP variants, and our extensive experiments demonstrate that ReasonCLIP not only substantially improves commonsense and compositional reasoning performance, but also enhances descriptive alignment. 
% %
% Furthermore, when integrated as a drop-in encoder into multimodal systems such as LLaVA and SDXL, ReasonCLIP consistently yields performance gains, establishing it as a strong reasoning-oriented CLIP-style backbone.
% %
% Our results show that the representation space of CLIP remains extensible, and large-scale reasoning supervision can expand its expressive boundaries, suggesting that reasoning-oriented data should be incorporated into the pretraining of CLIP-style backbones.
% %
% All datasets, models, and training scripts will be released publicly. 
% \NL{Including our main contributions figure on the 1st page would help draw readers’ attention and improve readability at a glance.}
\end{abstract}

==> sec/1-intro.tex <==
\section{Introduction}
% ===== Refined Naufal =====
% \NL{===Refined version===}

% ==== Version 2 =====
% Motivation
Contrastive Language-Image Pretraining (CLIP) \cite{radford2021learning} has emerged as a foundational vision-language model that aligns image and text representations through large-scale contrastive learning. Since its introduction, CLIP-style visual encoders \cite{zhai2023sigmoid,sun2024eva,tschannen2025siglip} have become the default backbone for multimodal systems, including Multimodal Large Language Models (MLLMs) \cite{li2023blip,alayrac2022flamingo,li2024llava,Qwen3-VL}. %and Text-to-Image (T2I) frameworks \cite{podellsdxl,flux2024}. 
Despite their widespread adoption, most CLIP models are pretrained on large-scale \emph{descriptive} image-text datasets \cite{jia2021scaling,schuhmann2021laion}, where supervision primarily encourages semantic correspondence rather than structured reasoning over visual content. While highly effective for retrieval, such training is not explicitly designed to support visually grounded reasoning~\cite{jiang2025mme,zhang2024mmvp,xu2025visulogic,kamath2026scale,cui2024more,wan2022bridging}.
% Why standard contrastive training is not enough

Advanced MLLMs increasingly require capabilities beyond descriptive alignment, including compositional reasoning~\cite{johnson2017clevr,hudson2019gqa}, commonsense inference~\cite{yue2024mmmu,hu2025video}, and multi-step understanding~\cite{wei2022chain,xu2024llava}, when processing complex and diverse real-world scenarios.
%\BZ{TODO: }Advanced multimodal systems increasingly require capabilities beyond descriptive alignment, including compositional reasoning \cite{johnson2017clevr,hudson2019gqa}, commonsense inference \cite{yue2024mmmu,hu2025video}, and multi-step understanding \cite{wei2022chain,xu2024llava}.
%
However, as summarized in Tab.~\ref{tab:main: model_compare}, recent CLIP advances largely focus on scaling descriptive data \cite{datacomp,xu2023demystifying,zhai2023sigmoid} or refining architectures \cite{zhang2024long,sun2024eva,bolyaperception,kwon2023efficient}. This emphasis creates a mismatch between pretraining objectives and reasoning-oriented downstream demands, questioning whether descriptive alignment alone is sufficient for visually grounded reasoning.

% Our solution
Motivated by this gap, we revisit CLIP and investigate whether its representation space can be extended through reasoning-oriented continual pretraining \emph{without modifying its architecture}. 
As illustrated in Fig.~\ref{fig:teaser}, we propose ReasonCLIP-58M, a two-stage continual pretraining framework to train a family of CLIP-style visual encoders with over 58.9M visually grounded commonsense reasoning samples. This design progressively enhances reasoning capacity while explicitly preserving the model’s original descriptive alignment.
% As illustrated in Fig.~\ref{fig:teaser}, we propose \textbf{ReasonCLIP-58M}, a two-stage training framework that leverages \textbf{58.9M} visually grounded commonsense reasoning samples to progressively enhance reasoning capacity while preserving the original descriptive alignment.

% As illustrated in Fig.~\ref{fig:teaser}, we introduce \textbf{ReasonCLIP-58M}, a multi-stage training framework leveraging \textbf{58.9M} visually grounded commonsense reasoning samples to progressively enhance reasoning capacity while preserving descriptive alignment.
% a multi-stage training framework leveraging \textbf{58.9M} visually grounded commonsense reasoning samples to progressively enhance reasoning capacity while preserving descriptive alignment.

% Summarized methodology [Training > Dataset]
In the first stage, we incrementally introduce reasoning signals to preserve the model’s original descriptive alignment while enhancing its sensitivity to visually grounded inference. To support this, we construct ReasonLite-42M, which augments descriptive captions with visually verifiable reasoning statements.
In the second stage, we strengthen supervision with structured category-level signals using ReasonPro-16M, a dataset spanning five visually grounded reasoning types: \textit{Spatial/Geometric, Attribute/State, Creature/Action, Temporal/Phase, and Intuitive Physics}. This stage encourages the model to explicitly distinguish and organize diverse reasoning patterns within its visual representation space.
%
% In the first stage, we introduce reasoning signals incrementally to preserve the model’s original descriptive alignment while enhancing its reasoning sensitivity.
% We construct \textbf{ReasonLite-42M}, which augments descriptive captions with visually verifiable reasoning statements and serves as supervision for this reasoning-aware alignment stage.
% % We construct \textbf{ReasonLite-42M}, which augments descriptive captions with visually verifiable reasoning statements and serves as supervision for the reasoning-aware alignment stage of our continual pretraining. 
% In the second stage, we strengthen reasoning supervision through structured category-level signals.
% We build \textbf{ReasonPro-16M}, a category-specific dataset spanning five visually grounded reasoning types: \textit{spatial/geometric, attribute/state, human/action, temporal/phase, and intuitive physics}. This dataset is used in a subsequent stage to introduce explicit category-level reasoning supervision, enabling the model to distinguish and organize these reasoning patterns within its visual representations.
%
% Summarized evaluation methodology
% \SC{TODO: more specific to illustrate training details and emphasis we train our new models} \NL{I revised, please check}
Using this progressive training strategy, we train CLIP and SigLIP variants at multiple scales to validate cross-architecture generality, resulting in ReasonCLIP and ReasonSigLIP models, respectively. To systematically evaluate reasoning ability, we introduce RCLIP-Bench, a diagnostic benchmark that decomposes visually grounded reasoning into three hierarchical levels: visual grounding, evidence awareness, and structured reasoning.
% \NL{I revised for explicit training detail and emphasis we train new model.}
% \hl{Using this progressive training strategy, we train multiple CLIP and SigLIP variants across model scales to validate cross-architecture generality. To systematically evaluate reasoning ability, we introduce \textbf{RCLIP-Bench}, a diagnostic benchmark that disentangles visually grounded reasoning into three levels: visual grounding, evidence awareness, and structured reasoning.} 
% Using this progressive continual pretraining strategy, we train multiple CLIP and SigLIP variants across model scales to validate cross-architecture generality. To evaluate visually grounded reasoning, we introduce \textbf{RCLIP-Bench}, a diagnostic benchmark that disentangles reasoning ability into three levels: visual grounding, evidence awareness, and structured visual reasoning.


\input{table/main_model_compare}

% Summarized results
Extensive experiments demonstrate that ReasonCLIP-58M consistently improves performance on visually grounded and compositional reasoning benchmarks across multiple backbones and model scales. Notably, reasoning-oriented continual pretraining also yields consistent gains in zero-shot retrieval tasks, suggesting that CLIP’s representation space remains highly extensible. Furthermore, when integrated as a drop-in backbone into MLLM, such as LLaVA-NeXT \cite{liu2024llavanext}, ReasonCLIP's encoder delivers stable performance gains without additional inference overhead.
% Summarized contribution
Our contributions are summarized as follows:
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]

\item \textbf{Explicit visually grounded commonsense reasoning supervision.} We introduce ReasonCLIP‑58M, a continual pretraining framework and datasets that injects visually grounded commonsense reasoning into CLIP-style encoders while preserving descriptive alignment and architectural compatibility.

\item \textbf{Two-stage reasoning-aware continual pretraining.} We design a structured two-stage training scheme that decouples reasoning enhancement from descriptive alignment preservation and enables organized reasoning patterns without degrading the original representation space.

\item \textbf{Reasoning-enhanced CLIP/SigLIP variants}. We train ReasonCLIP and ReasonSigLIP models at multiple scales that consistently improve visually grounded and compositional reasoning as well as zero-shot retrieval.

\item \textbf{Comprehensive evaluation and RCLIP-Bench.} We evaluate on diverse reasoning tasks and introduce RCLIP-Bench, which diagnoses visual grounding, evidence awareness, and structured visual reasoning.

% \item \textbf{Explicit visually grounded commonsense supervision for CLIP.} 
% We introduce ReasonCLIP-58M, a large-scale supervision framework that injects visually grounded commonsense reasoning directly into CLIP-style visual encoders through progressive continual pretraining, while preserving descriptive alignment and architectural compatibility.

% \item \textbf{Multi-stage reasoning-aware continual pretraining.}
% We design a structured training strategy that decouples reasoning enhancement from alignment preservation, enabling the visual encoder to acquire organized reasoning patterns without degrading its original representation quality.

% \item \textbf{Reasoning-enhanced visual encoders across architectures.}
% We train and release CLIP and SigLIP variants enhanced with visually grounded reasoning across multiple backbones and model scales, achieving consistent gains on reasoning benchmarks and zero-shot retrieval.

% \item \textbf{Comprehensive evaluation and a dedicated benchmark.}
% We perform a broad evaluation on visually grounded commonsense and compositional reasoning tasks, and introduce RCLIP-Bench, a benchmark that diagnoses model behavior across three levels of reasoning difficulty: visual grounding, evidence awareness, and structured visual reasoning, enabling precise analysis of where current models fail to reason over visual content.

\end{itemize}

% ==== Version 2 ===

% % Motivation
% Contrastive Language-Image Pretraining (CLIP) \cite{radford2021learning} has emerged as a vision-language foundation model that aligns image and text representations through large-scale contrastive learning. Since its introduction, CLIP-style visual encoders \cite{zhai2023sigmoid,sun2024eva, tschannen2025siglip} have become the de facto backbone in a wide range of multimodal systems, including Multimodal Large Language Models (MLLMs) \cite{li2023blip, alayrac2022flamingo, li2024llava, Qwen3-VL} and Text-to-Image generation (T2I) frameworks \cite{podellsdxl, flux2024}.
% Despite their widespread adoption, most existing CLIP models are trained on large-scale \emph{descriptive} image-text datasets \cite{jia2021scaling,schuhmann2021laion}, where the objective is to align visual content with natural-language descriptions. Although such supervision is highly effective for recognition and semantic alignment, it is primarily optimized for descriptive correspondence rather than structured reasoning over visual content.  % Revised by NFL. The teaser figure is moved to paragraph two to improve flow and structure (assuming the teaser revision is complete). 
%
% Despite their widespread adoption, as shown in Fig~\ref{fig:teaser}, existing CLIP models are predominantly trained on large-scale \emph{descriptive} image-text datasets \cite{jia2021scaling,schuhmann2021laion}, explicitly designed to inject \emph{visual grounded commonsense reasoning supervision directly into the visual encoder} of CLIP-style models remains largely unexplored. 
% NFL Comments: This version feels logically abrupt. I revised this and moved the mention of the teaser to the next paragraph, assuming that Fig. 1 has been changed. Feel free to give feedback. 

% Advanced multimodal systems increasingly demand capabilities that extend beyond description-level alignment, including compositional reasoning \cite{johnson2017clevr,hudson2019gqa}, commonsense inference \cite{yue2024mmmu,hu2025video}, and multi-step understanding \cite{wei2022chain,xu2024llava}. However, as summarized in Tab.~\ref{tab:main: model_compare}, recent advances in CLIP largely emphasize descriptive data scaling \cite{datacomp,xu2023demystifying,zhai2023sigmoid} and architectural refinement \cite{zhang2024long,sun2023eva,bolya2025perception,kwon2023efficient}. This sustained focus on descriptive alignment leaves a gap in modeling visually grounded reasoning. The resulting \textit{mismatch} between CLIP pretraining objectives and reasoning-oriented downstream demands suggests that descriptive alignment alone may be insufficient for visually grounded reasoning tasks. 
% \NL{TD: If we are unable to show downstream tasks, then we'll need to revise this.} % NFL: I refined this paragraph
%
% Advanced multimodal systems increasingly require capabilities that extend beyond description-level alignment, including compositional reasoning \cite{johnson2017clevr, hudson2019gqa}, commonsense inference \cite{yue2024mmmu, hu2025video}, and multi-step understanding \cite{wei2022chain, xu2024llava}. Meanwhile, Tab.~\ref{tab:main: model_compare} shows that advances in CLIP predominantly emphasize descriptive data engineering \cite{datacomp,xu2023demystifying,zhai2023sigmoid} and architectural refinement \cite{zhang2024long,sun2023eva,bolya2025perception,kwon2023efficient}. This growing \textit{mismatch} between CLIP's pretraining objectives and reasoning-oriented downstream demands suggests that descriptive alignment alone may be insufficient for visual-grounded reasoning tasks.

% % Summarized methodology
% We first construct \textbf{ReasonLite-42M}, which augments descriptive captions with visually verifiable reasoning statements. This phase introduces reasoning-aware alignment, allowing the model to develop general reasoning capability while retaining its original descriptive grounding. We then leverage \textbf{ReasonPro-16M}, a category-specific dataset covering 5 visual grounded reasoning categories: \textit{spatial/geometric, attribute/state, human/action, temporal/phase, and intuitive physics}. With explicit category supervision, the model is encouraged to distinguish and structure different reasoning patterns within its visual representations. 
% %
% We train multiple CLIP and SigLIP variants using this progressive continual pretraining strategy.
% %
% To support systematic evaluation of the visual grounding reasoning, we further introduce \textbf{RCLIP-Bench}, a dedicated benchmark that provides fine-grained, diagnostic evaluation across three levels of visual-grounded reasoning: visual grounding, evidence awareness, and visual grounded reasoning.

% \input{table/main_model_compare}



% Extensive experiments demonstrate that ReasonCLIP consistently improves performance on visual-grounded and compositional reasoning benchmarks across multiple backbones and model scales. Notably, reasoning-oriented continual pretraining also yields consistent gains across zero-shot retrieval 
% % \sout{and recognition} 
% tasks, suggesting that CLIP’s representation space remains highly extensible. Furthermore, when integrated as a drop-in backbone into MLLMs and T2I systems, ReasonCLIP delivers stable performance gains without additional inference overhead.
% Summarized contribution
% Our contributions are summarized as follows:
% \BZ{Updated this part.}
% \setlist{nolistsep}
% \begin{itemize}[noitemsep,label=\textperiodcentered,leftmargin=*]
% \item \textbf{Visual grounded reasoning framework.} 
% We introduce a progressive, reasoning-oriented continual pretraining framework that injects visual grounded commonsense reasoning supervision directly into CLIP-style \emph{visual encoders}, while explicitly preserving descriptive alignment and \emph{without modifying the original architecture}.

% \item \textbf{Reasoning-enhanced image encoders across backbones.}
% Based on the proposed framework and the ReasonCLIP-58M corpus, we train and release a suite of reasoning-enhanced image encoders spanning multiple CLIP/SigLIP backbones and model scales, enabling drop-in replacement in downstream systems with architectural compatibility preserved.

% \item \textbf{Comprehensive evaluation and a dedicated benchmark.}
% We conduct extensive experiments across visual-grounded commonsense and compositional reasoning benchmarks, and further verify transferability to zero-shot retrieval as well as downstream MLLMs and T2I systems.
% To support systematic evaluation of reasoning ability in CLIP-style architectures, we introduce \textbf{RCLIP-Bench}, a dedicated benchmark that diagnoses model failures across three levels of reasoning difficulty — visual grounding, evidence awareness, and visual-grounded reasoning, enabling precise identification of where and how a model's reasoning breaks down.

% \end{itemize}

% Despite their widespread adoption, existing CLIP models are predominantly trained on large-scale descriptive image–text datasets \cite{jia2021scaling,schuhmann2021laion}, where the objective is to align visual content with natural language captions. However, modern multimodal systems increasingly require capabilities that extend beyond description-level alignment, including compositional reasoning \cite{johnson2017clevr, hudson2019gqa}, commonsense inference \cite{yue2024mmmu, hu2025video}, and multi-step understanding \cite{wei2022chain, xu2024llava}. This growing mismatch between descriptive pretraining objectives and reasoning-oriented downstream demands raises a fundamental question: 

% Our solution
% In this work, we revisit CLIP from a foundation model perspective and ask whether its representation space can be systematically extended through large-scale reasoning-oriented continual pretraining without modifying its architecture. To this end, we introduce \textbf{ReasonCLIP}, a family of visual encoders trained on 58.9M automatically constructed perception-grounded reasoning samples.

% Summarized methodology
% \NL{TODO: Emphasize the multi-stage training proposal}
% Our approach follows a progressive multi-stage strategy. First, we construct \textbf{ReasonLite-42M}, an open-form reasoning dataset that augments descriptive captions with visually verifiable reasoning statements, enabling the model to acquire general reasoning awareness while preserving its original descriptive alignment. We then introduce \textbf{ReasonPro-16M}, a category-specific reasoning dataset that provides structured supervision across five perception-grounded reasoning types: \textit{spatial/geometric, attribute/state, human/action, temporal/phase, and intuitive physics}. Building on these datasets, we perform stage-wise continual pretraining that progressively injects reasoning capability into the visual encoder while maintaining architectural compatibility with CLIP and SigLIP \cite{tschannen2025siglip}.

% \noindent \NL{==== Original Version ====}

% % ======= Original Version ========
% Contrastive Language-Image Pretraining (CLIP) \cite{radford2021learning} is a vision foundational model, aligning image and text representations through contrastive learning.
% Since its release, CLIP-style visual encoders \cite{zhai2023sigmoid,sun2024eva, tschannen2025siglip} have become the de-facto choice \cite{tong2024cambrian} of vision backbone in diverse multimodal systems \cite{li2023blip, alayrac2022flamingo, podellsdxl, flux2024,li2024llava, Qwen3-VL}. 
% Existing CLIP models and their variants are primarily trained on large-scale \textit{descriptive image-text dataset} \cite{jia2021scaling,schuhmann2021laion}, with training objectives centered on aligning visual content with natural language descriptions. However, multimodal systems built upon such CLIP-style visual representations are increasingly required to handle tasks that demand compositional understanding \cite{johnson2017clevr, hudson2019gqa}, commonsense or deep reasoning \cite{yue2024mmmu, hu2025video}, and multi-step inference \cite{wei2022chain, xu2024llava}, etc. This \textit{mismatch} \cite{lovering2023training, fu2024blink, fu2025hidden, alam2026spatial} between training objectives and application requirements raises a critical question: \textbf{\textit{Are visual representations learned through descriptive alignment sufficient for downstream tasks that require reasoning?}}

% % Recent progress in reasoning MLLM has largely focused on enhancing the language-side inference process through three major paradigms: (1) multimodal chain-of-thought (CoT) methods \cite{xu2024llava}, which encourage step-by-step reasoning; (2) supervised reasoning fine-tuning \cite{} based on curated visual–reasoning datasets; and (3) reinforcement learning (RL) strategies \cite{yang2025r1,huang2025vision} inspired by Deeseek-R1 \cite{guo2025deepseek}. Despite these efforts, the improvements in reasoning MLLMs remain significantly smaller than those achieved in pure language models \cite{zhou2025r1}.



% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=\linewidth]{fig/Gemini_Generated_Image_yxs29yxs29yxs29y.png}
% %     \caption{TBD.}
% %     \SC{just a example by Gemini}
% %     \label{fig: teaser}
% % \end{figure}


% % Although recent studies have begun to explore enhancing CLIP models with common sense capabilities, such as modifying loss functions \cite{patel2024tripletclip}, xxxx \cite{} to improve visual representations, these approaches are conducted under the assumption that the visual encoder’s representation space remains largely stable, and primarily yield limited reasoning gains that are closely tied to dataset-specific patterns rather than deeper semantic understanding \cite{alhamoud2025vision}. When the CLIP visual encoder is trained at large scale with substantial representational changes, it remains unclear how well its original visual capabilities are preserved; how much intrinsic reasoning ability it can acquire; and how these changes affect reasoning performance in MLLMs.
% % Therefore, recent works have attempted to enhance CLIP's visual representations from several directions.
% Some approaches \cite{sun2023eva} focus on strengthening language alignment, for example by leveraging large language models to refine textual supervision \cite{huang2024llm2clip}, but their improvements are primarily driven by language-side enhancements.
% Others, such as Perception Encoder \cite{bolya2025perception}, improve perceptual quality through robust and scalable pretraining, revealing strong perceptual features from intermediate layers, yet they do not explicitly train the model to encode reasoning grounded in visual evidence.
% A separate line of work targets compositional reasoning, such as TripletCLIP \cite{patel2024tripletclip} and READ-CLIP \cite{kwon2025enhancing}, but these methods are typically fine-tuned on limited-scale datasets or evaluated under narrowly defined task settings \cite{dumpala2024sugarcrepe++, Alhamoud_2025_CVPR}, such as word swapping or replacement.



% % Recent works have begun to enhance CLIP’s visual representation, 1) Stronger text emb, like LLM2CLIP, Eva-CLIP 3) better Perception like Perception Encoder but not explicit reasoning 3) compostional reasoning \cite{patel2024tripletclip} but are fine-tuned on limited-scale data \cite{kwon2025enhancing} or under specific task settings \cite{dumpala2024sugarcrepe++, Alhamoud_2025_CVPR} such as word swapping and replacement. 

% % 不是让 CLIP 显式输出 reasoning chain，而是让它“在 embedding space 里 already know what matters for reasoning”。
% However, relatively little attention has been paid to developing CLIP’s \textbf{commonsense reasoning} % 
% % \footnote{This paper focuses on spatial, state, action, temporal, and intuitive physics reasoning, which aligns well with CLIP-style visual representations.}
% ability through large-scale training, which is essential for inducing substantial representational changes. To endow CLIP with stronger perception-grounded reasoning abilities and offload downstream reasoning to the visual encoding stage, we \textbf{continually pretrain} the \textbf{ReasonCLIP} family using a self-generated \textbf{58.9M} perception-grounded reasoning dataset. Our contributions are shown as follows:




% \SC{How to make these clear and one-to-one correspondence. Dataset-Stage-Results} 
% % \NL{If you have done this part, I will structure it.}

% a) In Section \ref{Sec: Dataset}, we construct a large-scale, reasoning-oriented pretraining dataset. Built upon our relabeled CC12M \cite{changpinyo2021conceptual} version, our dataset comprises two complementary subsets: \textbf{ReasonLite-42M}, which introduces perception-grounded visual reasoning signals to progressively enhance reasoning sensitivity while preserving descriptive alignment, and \textbf{ReasonPro-16M}, which provides more specific supervision across different reasoning categories.

% b) In Section \ref{Sec: Methodology}, we propose a stage-wise training framework to enhance CLIP’s \textbf{reasoning ability} while \textbf{preserving its architecture and descriptive representations}. The model is first continually pretrained on ReasonLite to acquire general reasoning awareness while retaining the visual descriptive capability, then further trained on ReasonPro to improve discrimination across reasoning patterns. We additionally fine-tune five LoRA adapters for different reasoning types and tasks. Finally, we replace the vision backbone by ReasonCLIP in existing multimodal systems. 

% c) In Section \ref{Sec: Experiments}, we train the ReasonCLIP family on top of \textbf{CLIP} and \textbf{SigLIP} models and conduct comprehensive evaluations. \SC{should we put the percentage here, we got 5\%-10\% higher on nearly all benchmarks} \NL{Yes, summarized consistent gain should be better for introduction.} Across all variants, ReasonCLIP consistently \textbf{outperforms} its corresponding pretrained base model in fundamental visual retrieval and descriptive alignment. It also achieves significant \textbf{gains} on commonsense and compositional reasoning benchmarks. Finally, when used as a vision backbone, ReasonCLIP provides stable performance improvements within both MLLMs and text-to-image generation systems.

% % The ReasonCLIP family is unified and comprehensive, and can be seamlessly integrated as a \textbf{plug-in replacement} for CLIP-style backbone in a wide range of downstream multimodal systems. 

% Beyond empirical performance gains, and grounded in widely adopted large-scale training practices, our study yields the following insights:
% \setlist{nolistsep}
% \begin{itemize}
% [noitemsep,leftmargin=*] 
%     \item CLIP’s representation space remains highly extensible, and even existing billion-scale data engineering efforts have not fully exhausted its potential.
%     \item Large-scale, perception-grounded reasoning continual pretraining not only enhances reasoning ability but also leads to improvements in fundamental visual representations.
%     \item Shifting perception-grounded reasoning abilities toward the visual encoding stage is beneficial for improving overall performance in multimodal systems.
% \end{itemize}

